Fast Algorithms for Separable Linear Programs

In numerical linear algebra, considerable effort has been devoted to obtaining faster algorithms for linear systems whose underlying matrices exhibit structural properties. A prominent success story is the method of generalized nested dissection~[Lipton-Rose-Tarjan'79] for separable matrices. On the other hand, the majority of recent developments in the design of efficient linear program (LP) solves do not leverage the ideas underlying these faster linear system solvers nor consider the separable structure of the constraint matrix. We give a faster algorithm for separable linear programs. Specifically, we consider LPs of the form $\min_{\mathbf{A}\mathbf{x}=\mathbf{b}, \mathbf{l}\leq\mathbf{x}\leq\mathbf{u}} \mathbf{c}^\top\mathbf{x}$, where the graphical support of the constraint matrix $\mathbf{A} \in \mathbb{R}^{n\times m}$ is $O(n^\alpha)$-separable. These include flow problems on planar graphs and low treewidth matrices among others. We present an $\tilde{O}((m+m^{1/2 + 2\alpha}) \log(1/\epsilon))$ time algorithm for these LPs, where $\epsilon$ is the relative accuracy of the solution. Our new solver has two important implications: for the $k$-multicommodity flow problem on planar graphs, we obtain an algorithm running in $\tilde{O}(k^{5/2} m^{3/2})$ time in the high accuracy regime; and when the support of $\mathbf{A}$ is $O(n^\alpha)$-separable with $\alpha \leq 1/4$, our algorithm runs in $\tilde{O}(m)$ time, which is nearly optimal. The latter significantly improves upon the natural approach of combining interior point methods and nested dissection, whose time complexity is lower bounded by $\Omega(\sqrt{m}(m+m^{\alpha\omega}))=\Omega(m^{3/2})$, where $\omega$ is the matrix multiplication constant. Lastly, in the setting of low-treewidth LPs, we recover the results of [DLY,STOC21] and [GS,22] with significantly simpler data structure machinery.

==> tree_operator/soln_data_struct.tex <==
\section{Solution data structures} \label{sec:soln-data-struct}

\TODO{..}
We combine the previous parts on maintaing the implicit primal and dual solutions, and maintaining the explicit approximations, to form the overall data structure needed for the IPM.

\begin{restatable}[Slack maintenance]{theorem}{SlackMaintain}
	\label{thm:SlackMaintain}
	%
	Given a modified planar graph $G$ with $m$ edges and its separator tree $\ct$ with height $\eta$,
	the randomized data structure \textsc{MaintainSlack} (\cref{alg:slack-maintain-main})
	implicitly maintains the slack solution $\vs$ undergoing IPM changes,
	and explicitly maintains its approximation $\os$,
	and supports the following procedures with high probability against an adaptive adversary:
	\begin{itemize}
		\item $\textsc{Initialize}(G,\vs^{\init} \in\R^{m},\vv\in \R^{m}, \vw\in\R_{>0}^{m},\epsilon_{\mproj}>0,\overline{\epsilon}>0)$:
		Given a graph $G$, initial solution $\vs^{\init}$, initial direction $\vv$, initial weights $\vw$,
		target step accuracy $\epsilon_{\mproj}$ and target approximation accuracy
		$\overline{\epsilon}$, preprocess in $\widetilde{O}(m \epsilon_{\mproj}^{-2})$ time, 
		and set the representations $\vs \leftarrow \vs^{\init}$ and $\ox \leftarrow \vs$.
		
		\item $\textsc{Reweight}(\vw\in\R_{>0}^{m},$ given implicitly as a set of changed weights): 
		Set the current weights to $\vw$ in $\widetilde{O}(\epsilon_{\mproj}^{-2}\sqrt{mK})$ time,
		where $K$ is the number of coordinates changed in $\vw$.
		
		\item $\textsc{Move}(\alpha\in\mathbb{R},\vv\in\R^{m} $ given implicitly as a set of changed coordinates): 
		Implicitly update  $\vs \leftarrow \vs+\alpha\mw^{-1/2}\widetilde{\mproj}_{\vw} \vv$ for some
		$\widetilde{\mproj}_{\vw}$ with	$\|(\widetilde{\mproj}_{\vw} -\mproj_{\vw}) \vv \|_2 \leq\eta\epssc \norm{\vv}_2$,
		and $\widetilde{\mproj}_{\vw} \vv \in \range{\mb}$. 
		The total runtime is $\widetilde{O}(\epsilon_{\mproj}^{-2}\sqrt{mK})$ where $K$ is the number of coordinates changed in $\vv$.
		
		\item $\textsc{Approximate}()\rightarrow\R^{m}$: Return the vector $\os$
		such that $\|\mw^{1/2}(\os-\vs)\|_{\infty}\leq\overline{\epsilon}$
		for the current weight $\vw$ and the current vector $\vs$. 
		
		\item $\textsc{Exact}()\rightarrow\R^{m}$: 
		Output the current vector $\vs$ in $\O(m \epssc^{-2})$ time.
	\end{itemize}
	Suppose $\alpha\|\vv\|_{2}\leq\beta$ for some $\beta$ for all calls to \textsc{Move}.
	Suppose in each step, \textsc{Reweight}, \textsc{Move} and \textsc{Approximate} are called in order. Let $K$ denote the total number of coordinates changed in $\vv$ and $\vw$ between the $(k-1)$-th and $k$-th \textsc{Reweight} and \textsc{Move} calls. Then at the $k$-th \textsc{Approximate} call,
	\begin{itemize}
		\item the data structure first sets $\os_e\leftarrow \vs^{(k-1)}_e$ for all coordinates $e$ where $\vw_e$ changed in the last \textsc{Reweight}, then sets $\os_e\leftarrow \vs^{(k)}_e$ for $O(N_k\defeq 2^{2\ell_{k}}(\frac{\beta}{\overline{\epsilon}})^{2}\log^{2}m)$ coordinates $e$, where $\ell_{k}$ is the largest integer
		$\ell$ with $k=0\mod2^{\ell}$ when $k\neq 0$ and $\ell_0=0$. 
		\item The amortized time for the $k$-th \textsc{Approximate} call
		is $\widetilde{O}(\epsilon_{\mproj}^{-2}\sqrt{m(K+N_{k-2^{\ell_k}})})$.
	\end{itemize}
	
\end{restatable}


\begin{restatable}[Flow maintenance]{theorem}{FlowMaintain}
	%
	\label{thm:FlowMaintain}
	Given a modified planar graph $G$ with $m$ edges and its separator tree $\ct$ with height $\eta$,
	the randomized data structure \textsc{MaintainFlow} (\cref{alg:flow-maintain-main})
	implicitly maintains the flow solution $\vf$ undergoing IPM changes,
	and explicitly maintains its approximation $\of$, 
	and supports the following procedures with high probability against an adaptive adversary:
	\begin{itemize}
		\item
		$\textsc{Initialize}(G,\vf^{\init} \in\R^{m},\vv \in \R^{m}, \vw\in\R_{>0}^{m},\epsilon_{\mproj}>0,
		\overline{\epsilon}>0)$: Given a graph $G$, initial solution $\vf^\init$, initial direction $\vv$, 
		initial weights $\vw$, target step accuracy $\epsilon_{\mproj}$,
		and target approximation accuracy $\overline{\epsilon}$, 
		preprocess in $\widetilde{O}(m \epsilon_{\mproj}^{-2})$ time and set the internal representation $\vf \leftarrow \vf^{\init}$ and $\of \leftarrow \vf$.
		%
		\item $\textsc{Reweight}(\vw\in\R_{>0}^{m}$ given implicitly as a set of changed weights): Set the current weights to $\vw$ in
		$\widetilde{O}(\epsilon_{\mproj}^{-2}\sqrt{mK})$ time, where $K$ is
		the number of coordinates changed in $\vw$.
		%
		\item $\textsc{Move}(\alpha\in\mathbb{R},\vv\in\R^{m}$ given
		implicitly as a set of changed coordinates): 
		Implicitly update
		$\vf \leftarrow \vf+ \alpha \mw^{1/2}\vv - \alpha \mw^{1/2} \widetilde{\mproj}'_{\vw} \vv$ for
		some $\widetilde{\mproj}'_{\vw} \vv$, 
		where 
		$\|\widetilde{\mproj}'_{\vw} \vv - \mproj_{\vw} \vv \|_2 \leq O(\eta \epssc) \norm{\vv}_2$ and
		$\mb^\top \mw^{1/2}\widetilde{\mproj}'_{\vw}\vv= \mb^\top \mw^{1/2} \vv$.
		The runtime is $\widetilde{O}(\epsilon_{\mproj}^{-2}\sqrt{mK})$, where $K$ is
		the number of coordinates changed in $\vv$.
		%
		\item $\textsc{Approximate}()\rightarrow\R^{m}$: Output the vector
		$\of$ such that $\|\mw^{-1/2}(\of-\vf)\|_{\infty}\leq\overline{\epsilon}$ for the
		current weight $\vw$ and the current vector $\vf$. 
		%
		\item $\textsc{Exact}()\rightarrow\R^{m}$: 
		Output the current vector $\vf$ in $\O(m \epssc^{-2})$ time.
	\end{itemize}
	Suppose $\alpha\|\vv\|_{2}\leq\beta$ for some $\beta$ for all calls to \textsc{Move}.
	Suppose in each step, \textsc{Reweight}, \textsc{Move} and \textsc{Approximate} are called in order. Let $K$ denote the total number of coordinates changed in $\vv$ and $\vw$ between the $(k-1)$-th and $k$-th \textsc{Reweight} and \textsc{Move} calls. Then at the $k$-th \textsc{Approximate} call,
	\begin{itemize}
		\item the data structure first sets $\of_e\leftarrow \vf^{(k-1)}_e$ for all coordinates $e$ where $\vw_e$ changed in the last \textsc{Reweight}, then sets $\of_e\leftarrow \vf^{(k)}_e$ for $O(N_k\defeq 2^{2\ell_{k}}(\frac{\beta}{\overline{\epsilon}})^{2}\log^{2}m)$ coordinates $e$, where $\ell_{k}$ is the largest integer
		$\ell$ with $k=0\mod2^{\ell}$ when $k\neq 0$ and $\ell_0=0$. 
		\item The amortized time for the $k$-th \textsc{Approximate} call
		is $\widetilde{O}(\epsilon_{\mproj}^{-2}\sqrt{m(K+N_{k-2^{\ell_k}})})$.
	\end{itemize}
\end{restatable}


\begin{algorithm}
	
	\caption{Implementation of Robust Interior Point Method\label{algo:IPM_impl}}
	
	\begin{algorithmic}[1]
		
		\Procedure{$\textsc{CenteringImpl}$}{$\ma,\phi,\vx,\vs,t_{\mathrm{start}},t_{\mathrm{end}}$}
		
		\State $\mathcal{X}, \mathcal{S}$: data structures for primal and slack maintenance 
		\Comment \cref{thm:SlackMaintain,thm:FlowMaintain}
		
		\State $\alpha \defeq \frac{1}{2^{20}\lambda}, \lambda \defeq 64\log(256n^{2})$
		
		\State $t\leftarrow t_{\mathrm{start}}$, $\ox\leftarrow\vx,\os\leftarrow\vs,\ot\leftarrow t$, $\mw\leftarrow\nabla^{2}\phi(\ox)^{-1}$
		\Comment variable initialization
		\State $\vv_{i} \leftarrow \sinh(\lambda\gamma^{\ot}(\ox,\os)_{i})$ for all $i \in [n]$
		
		\Comment data structure initialization
		\State $\mathcal{X}.\textsc{Initalize}(\vx,\vv, \mw,\epssc=O(\alpha/\log n),\overline{\epsilon}=\alpha)$   
		\Comment choose $\epssc$ so $\eta\epssc \leq \alpha$ in \cref{thm:SlackMaintain} 
		\State $\mathcal{S}.\textsc{Initalize}(\ot^{-1}\vs,\vv, \mw,\epssc=O(\alpha/\log n),\overline{\epsilon}=\alpha)$ 
		\Comment and $O(\eta\epssc) \leq \alpha$ in \cref{thm:FlowMaintain}
		
		\While{$t\geq t_{\mathrm{end}}$}
		
		\State $t\leftarrow\max\{(1-\frac{\alpha}{\sqrt{n}})t, t_{\mathrm{end}}\}$
		
		\State Update $h=-\alpha/\|\cosh(\lambda\gamma^{\ot}(\ox,\os))\|_{2}$
		\Comment $\gamma$ as defined in \cref{eq:mu_t_def}\label{line:step_given_begin_impl}
		
		\State Update the diagonal weight matrix $\mw=\nabla^{2}\phi(\ox)^{-1}$\label{line:step_given_3_impl}
		
		\State $\mathcal{X}.\textsc{Reweight}(\mw)$ \Comment update the implicit representation of $\vx$ with new weights
		\State $\mathcal{S}.\textsc{Reweight}(\mw)$ \Comment update the implicit representation of $\vs$ with new weights
		
		\State $\vv_{i} \leftarrow \sinh(\lambda\gamma^{\ot}(\ox,\os)_{i})$ for all $i$ where $\ox_i$ or $\os_i$ has changed \label{line:step_given_end_impl} 
		\Comment update direction $\vv$
		
		\State $\mathcal{F}.\textsc{Move}(h,\vv)$
		\Comment  Update $\vx\leftarrow\vx+h\mw^{1/2}\vv - h \mw^{1/2} \tx$ 
		with $\tx \approx \mproj_{\vw} \vv$ 
		
		\State $\mathcal{S}.\textsc{Move}(h,\vv)$ \Comment Update $\vs\leftarrow\vs+\ot h\mw^{-1/2}\ts$ with $\ts \approx\mproj_{\vw} \vv$
		
		\State $\ox\leftarrow\mathcal{F}.\textsc{Approximate}()$ \Comment Maintain $\ox$ such that $\|\mw^{-1/2}(\ox-\vx)\|_{\infty}\leq\alpha$
		
		\State  $\os\leftarrow\bar{t}\mathcal{S}.\textsc{Approximate}()$ \Comment Maintain $\os$ such that  $\|\mw^{1/2}(\os-\vs)\|_{\infty}\leq\ot\alpha$
		
		\label{line:step_user_end_impl}
		
		\If {$|\ot-t|\geq\alpha\ot$} 
		\State $\vs\leftarrow \ot\mathcal{S}.\textsc{Exact}()$
		\State $\ot\leftarrow t$ 
		\State  $\mathcal{S}.\textsc{Initalize}(\ot^{-1}\vs, \vv, \mw,\epssc=O(\alpha/\log n),\overline{\epsilon}=\alpha)$ 
		%\State  $\mathcal{F}.\textsc{Initalize}(G,\mathcal{F}.\textsc{Exact}(), \vv, \mw,\epssc=\alpha,\overline{\epsilon}=\alpha)$
		%\TODO{don't think we need to reinitialize F}
		\EndIf 
		
		\EndWhile
		
		\State \Return $(\mathcal{F}.\textsc{Exact}(),\ot\mathcal{S}.\textsc{Exact}())$\label{line:step_user_output_impl}
		
		\EndProcedure
		
	\end{algorithmic}
	
\end{algorithm}


We first prove a lemma about how many coordinates change in $\vw$ and $\vv$ in each step. This is useful for bounding the complexity of each iteration.
\begin{lemma}\label{lem:cor_change}
	When updating $\vw$ and $\vv$ at the $(k+1)$-th step of the $\textsc{CenteringImpl}$ algorithm,
	$\vw$ and $\vv$ change in $O(2^{2\ell_{k-1}}\log^{2}m+2^{2\ell_{k}}\log^{2}m)$ coordinates, where $\ell_{k}$
	is the largest integer $\ell$ with $k \equiv 0\mod2^{\ell}$.
\end{lemma}
\begin{proof}
	Since both $\vw$ and $\vv$ are an entry-wise function of $\ox,\os$ and $\ot$, we need to examine these variables.
	First, $\ot$ changes every $\O(\sqrt{n})$ steps, and when $\ot$ changes, every coordinate of $\vw$ and $\vv$ changes.
	Over the entire \textsc{CenteringImpl} run, $\ot$ changes $\O(1)$ number of times, so we may incur an additive $\O(n)$ term overall, and assume $\ot$ does not change for the rest of the analysis.
	
	By \cref{thm:IPM}, we have $h\|\vv\|_2 = O(\frac{1}{\log m})$ at all steps. So we apply \cref{thm:SlackMaintain}  and \cref{thm:FlowMaintain} both with parameters $\beta = O(\frac{1}{\log m})$ and $\overline{\epsilon}=\alpha=\Theta(\frac{1}{\log m})$. We use their conclusions in the following argument.
	Let the superscript $^{(k)}$ denote the variable at the end of the $k$-th step.
	
	By definition, $\vw^{(k+1)}$ is an entry-wise function of $\ox^{(k)}$, and recursively, $\ox^{(k)}$ is an entry-wise function of $\vw^{(k)}$.
	%Because $\vw^{(k+1)}_i$ differs from $\vw^{(k)}_i$ only when $\ox^{(k)}_i$ is updated at the $k$-th step, 
	We first prove inductively that at step $k$, $O(2^{2\ell_{k}}\log^{2}m)$ coordinates of $\ox$ change to $\vx^{(k)}$ where $\vx^{(k)}$ is the exact solution, and there are no other changes. This allows us to conclude that $\vw^{(k+1)}$ differ from $\vw^{(k)}$ on $O(2^{2\ell_{k}} \log^2 m)$ coordinates.
	
	In the base case at step $k=1$, because $\vw^{(1)}$ is equal to the initial weights $\vw^{(0)}$, 
	only $O(2^{2\ell_{1}}\log^{2}m)$ coordinates $\ox_e$ change to $\vx^{(1)}_e$.
	%
	Suppose at step $k$, a set $S$ of $O(2^{2\ell_{k}}\log^{2}m)$ coordinates of $\ox$ change; that is, $\ox|_S$ is updated to $\vx^{(k)}|_S$, and there are no other changes. 
	Then at step $k+1$, by definition, $\vw^{(k+1)}$ differ from $\vw^{(k)}$ exactly on $S$, 
	and in turn, $\ox^{(k+1)}|_S$ is set to $\vx^{(k)}|_S$ again (\cref{line:D-induced-ox-change} of \cref{algo:maintain-vector}). 
	In other words, there is no change from this operation. 
	Then, $O(2^{2\ell_{k+1}}\log^{2}m)$ additional coordinates $\ox_e$ change to $\vx^{(k+1)}_e$.
	
	Now, we bound the change in $\os$: \cref{thm:SlackMaintain} guarantees that in the $k$-th step, there are $O(2^{2\ell_{k}}\log^{2}m)+D$ coordinates in $\os$ that change, where $D$ is the number of changes between $\vw^{(k-1)}$ and $\vw^{(k)}$ and is equal to $O(2^{2\ell_{k-1}} \log^2 m)$ as shown above.
	
	Finally, $\vv^{(k+1)}$ is an entry-wise function of $\ox^{(k)}$ and $\os^{(k)}$, so we conclude that $\vv^{(k+1)}$ and $\vv^{(k)}$ differ on at most $O(2^{2\ell_{k}}\log^{2}m) + 2 \cdot O(2^{2\ell_{k-1}}\log^{2}m)$ coordinates.
\end{proof}

